Weakly supervised 3D Reconstruction with Adversarial Constraint

Supervised 3D reconstruction has witnessed a significant progress through the use of deep neural networks. However, this increase in performance requires large scale annotations of 2D/3D data. In this paper, we explore inexpensive 2D supervision as an alternative for expensive 3D CAD annotation. Specifically, we use foreground masks as weak supervision through a raytrace pooling layer that enables perspective projection and backpropagation. Additionally, since the 3D reconstruction from masks is an ill posed problem, we propose to constrain the 3D reconstruction to the manifold of unlabeled realistic 3D shapes that match mask observations. We demonstrate that learning a log-barrier solution to this constrained optimization problem resembles the GAN objective, enabling the use of existing tools for training GANs. We evaluate and analyze the manifold constrained reconstruction on various datasets for single and multi-view reconstruction of both synthetic and real images.

==> 4-implementation.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\linewidth]{network/network2}
    \caption{Visualization of \wsgan~ network structure. Our network encodes a set of images into a latent variable. Then, the latent variable is decoded into a voxel representation of 3D shape. Perspective Raytrace Pooling layer renders this 3D shape into 2D occupancy map, allowing us to give mask supervision. Additionally, discriminator takes the generated voxel as an input, filliing the missing information of the 3D shape distribution learned from unlabeled 3D models.}
    \label{fig:network}
    \vspace{-10pt}
\end{figure*}

\vspace{-3pt}
\paragraph{Network}
We implemented \mcrecon with a symbolic math neural network library~\cite{theano}. For the generator, we use the Deep-Residual-GRU network proposed by
Choy \etal\cite{3dr2n2}, which uses a 2D convolutions with and 3D decoder with
residual connections across layers and GRUs for RNN implementation.
The schematics of \mcrecon is in Fig.~\ref{fig:network}. We used RGB images of size $127^2$ as an input and the voxel reconstruction
of size $32^3$ ($N_v=32$) as an output. For the \raytracinglayer, we use the silhouette of size $127^2$. Finally, for the discriminator, we stacked 3D convolutions
and 3D poolings until the size of activation becomes $2\times 2\times 2$ and flatten to feed the activations to a fully connected layer followed by a
softmax layer. The details of the network architecture are in the supplementary
material.

\vspace{-5pt}
\paragraph{Optimization}
Discriminator training is notoriously difficult \cite{dcgan, improvedtechforgan, affgan} and barrier training of the \mcreconfull was not an exception. Inherently, the discriminator training involves computing $\log q/p$ which can
cause divergence if support of $p$ does not overlap with the support of $q$ ($p$ is the distribution of $x^\star$ and $q$ is the distribution of $\hat{x}$).
To prevent such case, we followed the instance noise technique by S{\o}nderby \etal\cite{affgan} which smooths the probability space to make the support of $p$ infinite.
In addition, we used the update rule in \cite{3dgan} and train the
discriminator only if its prediction error becomes larger than 20\%. This technique makes the discriminator imperfect and prevents saturation of $g$. Finally,
we use different learning rate for $f$ and $g$:
$10^{-2}$ for $\theta_f$ and $10^{-4}$ for $\theta_g$ and reduce the learning
rate by the factor of 10 after 10,000 and 30,000 iterations. 
We train the network over 40,000 iterations using ADAM~\cite{adam} with batch
size 8. We used loss balancing hyper-parameter $\lambda=0.01$ for all experiments.
% For multi view training, we randomly choose the number of input images between 1 to 5.

==> theory.tex <==
We want to train a network to reconstruct a 3D shape given a set of single or
multiple view image(s) without ground-truth 3D models associated to the
image(s). Unlike \cite{singleviewproj} which requires a large number of
2D foreground masks, we focus on a single foreground segmentation or few since
(1) dense viewpoint annotations are difficult to generate unless 3D shape
annotation is given and (2) Structure from Motion can generate accurate 3D
shapes in presence of dense viewpoint.

The inputs are one or sparse views of image(s), corresponding foreground
mask(s) and camera parameter(s). At test time, we only require query images,
and optionally take their camera parameters to
further improve the quality of the reconstruction.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{network/diagram}
    \caption{Weakly Supervised Generate Adversarial Network. $u, v$ are image(s)
        and foreground segmentation mask(s) respectively. $z$ is the latent
        variable and $x$ is the generated 3D reconstruction. The $v$ provides
        weak supversion to $x$ using projective transformation. Given the unlabeled 3D
        shapes $\hat{x}$, the discriminator $D(\cdot)$ learns the manifold
    of 3D shapes.} \label{fig:diagram}
\end{figure}

In this weakly supervised setting, where domain of input $u$ and weak
supervision $v$ are different from that of target $x$, the distribution of
data $p(x)$ in the target space can guide the weakly supervised
generation $q(x)$. More precisely, input image $u$ and corresponding mask $v$
are given but we do not have labeled 3D shape $x$, and we have access to a
large pool of 3D shapes $\hat{x} \sim p(x)$. Simply by leveraging the
distribution of 3D shapes $p(x)$, we can guide the weakly supervised
reconstruction (Section~\ref{sect:gan-subsection}).

However, a certain category of object might be more prevalent in the pool of
unlabeld 3D shapes $\hat{x}$ whereas it might be scarce in the input image-mask
pair $(u, v)$. In such general setting, there is no guarantee for convergence or global
optimality which exist for GAN~\cite{gan}. We first prove the existence of
global optimality and convergence of Weakly Supervised GAN for different modality or
distribution.


\subsection{Global Optimality of Weakly Supervised GAN}
\label{sec:theory}

Let $c$ be the category of an object. The target category distribution $p_c = p(c)$
may be different from the input category distribution $q_c = q(c)$ since $p(x)$ is
unlabeled data. Then, $q(x | c)q(c)$ cannot match $p(x|c)p(c)$.

\begin{corollary}
    By the proposition 1 in \cite{gan}, for fixed $G$, the optimal discriminator $D$ is

    \begin{equation}
        D^* = \frac{p(x | c)p(c)}{p(x|c)p(c) + q(x|c)q(c)}
    \end{equation}
\end{corollary}

Let $V(G, D)$ be $\mathbb{E}_{x \sim p} \log D(x) + \mathbb{E}_{x
\sim q} \log(1 - D(x))$, the objective function of GAN. Following \cite{gan},
we denote $C(G) = V(G, D^*)$.

\begin{theorem} \label{theorem:global_min}
    The global minimum of the criterion $C(G)$ is achieved if and only if
    $p(x|c) = q(x|c)$ and the value at the minimum is
    $C^* = -\log 4 + 2D_{JS}(\infdivx{p_c}{q_c})$.
\end{theorem}

\begin{sketch}
    At $q(x|c) = p(x|c)$, $D^*=\frac{p_c}{p_c + q_c}$ and we substitute $D$
    with $D^*$ to get $C(G)$. Then, first subtract and add the optimal value
    $C^*$ to $C(G)$. Factoring the terms, we get
    $\mathbb{E}_{p_c}D_{KL}\left(\infdivx{p(x|c)}{\frac{p(x|c) p_c + q(x|c) q_c}{p_c + q_c}}\right)$
    for $p_c$ and similar result for $q_c$. Since
    $D_{KL}(\infdivx{\cdot}{\cdot}) \ge 0$, $C^* \le C(G)$. The detailed proof
    is in the supplementary material.

    % For $q(x|c) = p(x|c)$, the optimal discriminator $D^* = \frac{p(c)}{p(c) + q(c)}$.
    % We denote $p(c)$ and $q(c)$ as $p_c$ and $q_c$ respectively. If we add and substract $2D_{JS}(\infdivx{p_c}{q_c})$ to $C(G)$,

    % \begin{align}
    %     C(G) & = \mathbb{E}_{p_c}\mathbb{E}_p \log \frac{p(x|c) p_c}{p(x|c) p_c + q(x|c) q_c} + \mathbb{E}_{q_c}\mathbb{E}_q \log \frac{q(x|c)q_c}{p(x|c)p_c + q(x|c)q_c}\\
    %     & = 2D_{JS}(\infdivx{p_c}{q_c}) + \mathbb{E}_{p_c}\mathbb{E}_p \log \frac{p(x|c) (p_c + q_c)}{2(p(x|c) p_c + q(x|c) q_c)} + \mathbb{E}_{q_c}\mathbb{E}_q \log \frac{q(x|c)(p_c + q_c)}{2(p(x|c)p_c + q(x|c)q_c)} \\
    %     & = -\log 4 + 2D_{JS}(\infdivx{p_c}{q_c}) + \mathbb{E}_{p_c}\mathbb{E}_p \log \frac{p(x|c) (p_c + q_c)}{2(p(x|c) p_c + q(x|c) q_c)} + \mathbb{E}_{q_c}\mathbb{E}_q \log \frac{q(x|c)(p_c + q_c)}{2(p(x|c)p_c + q(x|c)q_c)} \\
    %     & = -\log 4 + 2D_{JS}(\infdivx{p_c}{q_c}) + \mathbb{E}_{p_c}D_{KL}(\infdivx{p(x|c)}{\frac{p(x|c) p_c + q(x|c) q_c}{p_c + q_c}}) + \mathbb{E}_{q_c}D_{KL}(\infdivx{q(x|c)}{\frac{p(x|c) p_c + q(x|c) q_c}{p_c + q_c}}) \\
    %     & \ge -\log 4 + 2D_{JS}(\infdivx{p_c}{q_c})
    % \end{align}
\end{sketch}

By the proposition 2 in \cite{gan}, we can trivially show that the $q(x|c)$
converges to $p(x|c)$. Thus, when unlabeled target distribution is different
from the input distribution, we can show that the weakly supervised GAN may
converge to the global optimum.
Although we are optimizing $\theta_G$ in $q(x|c;\theta_G)$ using a neural
network rather than $q(x|c)$ directly, $G$ converges to a reasonable local
optimum in practice.

% However, practically, we model
% $q(x|c;\theta_G)$ using a neural network which can represent a limited family
% of distributions. Thus, the convergence might not be 

% However, as pointed out in \cite{gan}, we are
% optimizing $\theta_G$, which models a limited family of probability
% distributions so the optimization might fail but.

% To sum up, we use the perspective voxel raytrace pooling layer for and the
% combination of the 3D-Recurrent Reonstruction Neural Network~\cite{3dr2n2} as
% a Generator in a Generative Adversarial Netwokr framework To regularize the
% network to generate a realistic 3D shapes, we used the Generative Adversarial
% Network.

% As an extension, we present a feedback network which refines the reconstruction
% quality over iteration given camera parameter at test time in
% Section~\ref{sec:feedback}.



